What Does a Harness Buy? Tokens, Mostly

A coding agent is a language model inside a harness: the system prompt, the tools, and the context management that let a chat model work in a repository. Most of the engineering on these agents goes into the harness, and vendors and leaderboards credit it with score gains. Earlier studies have fixed the model and swapped the harness, but have not measured whether the swap changes the pass rate more than running the same harness again. We run seven models through three production harnesses, Claude Code, mini-SWE-agent, and OpenCode, on SWE-bench Verified and two benchmarks of other kinds, and rerun them unchanged. No harness leads consistently across models. Where the data can bound the difference between two harnesses, the bound is 2 to 5 points, and a harness swap changes about as many task outcomes as a rerun. The exceptions are harness effects in particular pairings of model and harness, whose direction changes with the model: OpenCode trails by 8 to 9 points on one model and leads by 14 on another. Cost differences between harnesses also depend on the model, from under 10% to 3 to 4 times. Which harness is better therefore has no answer apart from the model, and a harness difference should be reported next to a rerun.

==> numbers.tex <==
\makeatletter
\DeclareRobustCommand{\pn}[1]{\csname pn@#1\endcsname}
\expandafter\def\csname pn@cost.dsflash.CC.cny\endcsname{0.98}
\expandafter\def\csname pn@cost.dsflash.CC.hitpct\endcsname{99}
\expandafter\def\csname pn@cost.dsflash.CC.outk\endcsname{94}
\expandafter\def\csname pn@cost.dsflash.CC.steps\endcsname{104}
\expandafter\def\csname pn@cost.dsflash.CC.tokM\endcsname{8.7}
\expandafter\def\csname pn@cost.dsflash.OC.cny\endcsname{0.66}
\expandafter\def\csname pn@cost.dsflash.OC.hitpct\endcsname{99}
\expandafter\def\csname pn@cost.dsflash.OC.outk\endcsname{66}
\expandafter\def\csname pn@cost.dsflash.OC.steps\endcsname{88}
\expandafter\def\csname pn@cost.dsflash.OC.tokM\endcsname{6.1}
\expandafter\def\csname pn@cost.dsflash.mini.cny\endcsname{1.02}
\expandafter\def\csname pn@cost.dsflash.mini.hitpct\endcsname{99}
\expandafter\def\csname pn@cost.dsflash.mini.outk\endcsname{76}
\expandafter\def\csname pn@cost.dsflash.mini.steps\endcsname{141}
\expandafter\def\csname pn@cost.dsflash.mini.tokM\endcsname{11.5}
\expandafter\def\csname pn@cost.glmflash.CC.cny\endcsname{1.81}
\expandafter\def\csname pn@cost.glmflash.CC.hitpct\endcsname{97}
\expandafter\def\csname pn@cost.glmflash.CC.outk\endcsname{68}
\expandafter\def\csname pn@cost.glmflash.CC.steps\endcsname{88}
\expandafter\def\csname pn@cost.glmflash.CC.tokM\endcsname{6.7}
\expandafter\def\csname pn@cost.glmflash.OC.cny\endcsname{0.56}
\expandafter\def\csname pn@cost.glmflash.OC.hitpct\endcsname{96}
\expandafter\def\csname pn@cost.glmflash.OC.outk\endcsname{26}
\expandafter\def\csname pn@cost.glmflash.OC.steps\endcsname{55}
\expandafter\def\csname pn@cost.glmflash.OC.tokM\endcsname{2.0}
\expandafter\def\csname pn@cost.glmflash.mini.cny\endcsname{0.97}
\expandafter\def\csname pn@cost.glmflash.mini.hitpct\endcsname{98}
\expandafter\def\csname pn@cost.glmflash.mini.outk\endcsname{31}
\expandafter\def\csname pn@cost.glmflash.mini.steps\endcsname{80}
\expandafter\def\csname pn@cost.glmflash.mini.tokM\endcsname{3.7}
\expandafter\def\csname pn@cost.hy4.CC.cny\endcsname{2.86}
\expandafter\def\csname pn@cost.hy4.CC.hitpct\endcsname{98}
\expandafter\def\csname pn@cost.hy4.CC.outk\endcsname{44}
\expandafter\def\csname pn@cost.hy4.CC.steps\endcsname{80}
\expandafter\def\csname pn@cost.hy4.CC.tokM\endcsname{5.1}
\expandafter\def\csname pn@cost.hy4.OC.cny\endcsname{2.41}
\expandafter\def\csname pn@cost.hy4.OC.hitpct\endcsname{97}
\expandafter\def\csname pn@cost.hy4.OC.outk\endcsname{38}
\expandafter\def\csname pn@cost.hy4.OC.steps\endcsname{67}
\expandafter\def\csname pn@cost.hy4.OC.tokM\endcsname{3.6}
\expandafter\def\csname pn@cost.hy4.mini.cny\endcsname{4.13}
\expandafter\def\csname pn@cost.hy4.mini.hitpct\endcsname{97}
\expandafter\def\csname pn@cost.hy4.mini.outk\endcsname{65}
\expandafter\def\csname pn@cost.hy4.mini.steps\endcsname{88}
\expandafter\def\csname pn@cost.hy4.mini.tokM\endcsname{6.6}
\expandafter\def\csname pn@dsflash.hard45.CC.hi\endcsname{61}
\expandafter\def\csname pn@dsflash.hard45.CC.k\endcsname{21}
\expandafter\def\csname pn@dsflash.hard45.CC.lo\endcsname{33}
\expandafter\def\csname pn@dsflash.hard45.CC.n\endcsname{45}
\expandafter\def\csname pn@dsflash.hard45.CC.pct\endcsname{47}
\expandafter\def\csname pn@dsflash.hard45.CC.seeds\endcsname{2}
\expandafter\def\csname pn@dsflash.hard45.CCvOC.b\endcsname{4}
\expandafter\def\csname pn@dsflash.hard45.CCvOC.c\endcsname{2}
\expandafter\def\csname pn@dsflash.hard45.CCvOC.diff\endcsname{+4.4}
\expandafter\def\csname pn@dsflash.hard45.CCvOC.hi\endcsname{+15.3}
\expandafter\def\csname pn@dsflash.hard45.CCvOC.lo\endcsname{-6.7}
\expandafter\def\csname pn@dsflash.hard45.CCvOC.n\endcsname{45}
\expandafter\def\csname pn@dsflash.hard45.CCvOC.p\endcsname{.69}
\expandafter\def\csname pn@dsflash.hard45.CCvmini.b\endcsname{1}
\expandafter\def\csname pn@dsflash.hard45.CCvmini.c\endcsname{2}
\expandafter\def\csname pn@dsflash.hard45.CCvmini.diff\endcsname{-2.2}
\expandafter\def\csname pn@dsflash.hard45.CCvmini.hi\endcsname{+6.2}
\expandafter\def\csname pn@dsflash.hard45.CCvmini.lo\endcsname{-10.5}
\expandafter\def\csname pn@dsflash.hard45.CCvmini.n\endcsname{45}
\expandafter\def\csname pn@dsflash.hard45.CCvmini.p\endcsname{1.00}
\expandafter\def\csname pn@dsflash.hard45.OC.hi\endcsname{57}
\expandafter\def\csname pn@dsflash.hard45.OC.k\endcsname{19}
\expandafter\def\csname pn@dsflash.hard45.OC.lo\endcsname{29}
\expandafter\def\csname pn@dsflash.hard45.OC.n\endcsname{45}
\expandafter\def\csname pn@dsflash.hard45.OC.pct\endcsname{42}
\expandafter\def\csname pn@dsflash.hard45.OC.seeds\endcsname{1}
\expandafter\def\csname pn@dsflash.hard45.dsh.cny\endcsname{1.04}
\expandafter\def\csname pn@dsflash.hard45.dsh.hi\endcsname{61}
\expandafter\def\csname pn@dsflash.hard45.dsh.k\endcsname{21}
\expandafter\def\csname pn@dsflash.hard45.dsh.lo\endcsname{33}
\expandafter\def\csname pn@dsflash.hard45.dsh.n\endcsname{45}
\expandafter\def\csname pn@dsflash.hard45.dsh.pct\endcsname{47}
\expandafter\def\csname pn@dsflash.hard45.dsh.steps\endcsname{111}
\expandafter\def\csname pn@dsflash.hard45.mini.hi\endcsname{63}
\expandafter\def\csname pn@dsflash.hard45.mini.k\endcsname{22}
\expandafter\def\csname pn@dsflash.hard45.mini.lo\endcsname{35}
\expandafter\def\csname pn@dsflash.hard45.mini.n\endcsname{45}
\expandafter\def\csname pn@dsflash.hard45.mini.pct\endcsname{49}
\expandafter\def\csname pn@dsflash.hard45.mini.seeds\endcsname{1}
\expandafter\def\csname pn@dsflash.hard45.minivOC.b\endcsname{4}
\expandafter\def\csname pn@dsflash.hard45.minivOC.c\endcsname{1}
\expandafter\def\csname pn@dsflash.hard45.minivOC.diff\endcsname{+6.7}
\expandafter\def\csname pn@dsflash.hard45.minivOC.hi\endcsname{+16.6}
\expandafter\def\csname pn@dsflash.hard45.minivOC.lo\endcsname{-3.6}
\expandafter\def\csname pn@dsflash.hard45.minivOC.n\endcsname{45}
\expandafter\def\csname pn@dsflash.hard45.minivOC.p\endcsname{.38}
\expandafter\def\csname pn@flip.hard45.harness.max\endcsname{27}
\expandafter\def\csname pn@flip.hard45.harness.median\endcsname{13}
\expandafter\def\csname pn@flip.hard45.harness.min\endcsname{7}
\expandafter\def\csname pn@flip.hard45.harness.n\endcsname{15}
\expandafter\def\csname pn@flip.hard45.model.max\endcsname{56}
\expandafter\def\csname pn@flip.hard45.model.median\endcsname{22}
\expandafter\def\csname pn@flip.hard45.model.min\endcsname{7}
\expandafter\def\csname pn@flip.hard45.model.n\endcsname{35}
\expandafter\def\csname pn@flip.hard45.rerun.ladder.max\endcsname{18}
\expandafter\def\csname pn@flip.hard45.rerun.ladder.median\endcsname{16}
\expandafter\def\csname pn@flip.hard45.rerun.ladder.min\endcsname{9}
\expandafter\def\csname pn@flip.hard45.rerun.ladder.n\endcsname{7}
\expandafter\def\csname pn@flip.hard45.rerun.max\endcsname{18}
\expandafter\def\csname pn@flip.hard45.rerun.median\endcsname{13}
\expandafter\def\csname pn@flip.hard45.rerun.min\endcsname{2}
\expandafter\def\csname pn@flip.hard45.rerun.n\endcsname{10}
\expandafter\def\csname pn@flip.pool447.harness.max\endcsname{16}
\expandafter\def\csname pn@flip.pool447.harness.median\endcsname{16}
\expandafter\def\csname pn@flip.pool447.harness.min\endcsname{9}
\expandafter\def\csname pn@flip.pool447.harness.n\endcsname{6}
\expandafter\def\csname pn@flip.pool447.model.max\endcsname{22}
\expandafter\def\csname pn@flip.pool447.model.median\endcsname{17}
\expandafter\def\csname pn@flip.pool447.model.min\endcsname{16}
\expandafter\def\csname pn@flip.pool447.model.n\endcsname{3}
\expandafter\def\csname pn@flip.pool447.rerun.max\endcsname{13}
\expandafter\def\csname pn@flip.pool447.rerun.median\endcsname{13}
\expandafter\def\csname pn@flip.pool447.rerun.min\endcsname{13}
\expandafter\def\csname pn@flip.pool447.rerun.n\endcsname{1}
\expandafter\def\csname pn@glmflash.hard45.CC.hi\endcsname{63}
\expandafter\def\csname pn@glmflash.hard45.CC.k\endcsname{22}
\expandafter\def\csname pn@glmflash.hard45.CC.lo\endcsname{35}
\expandafter\def\csname pn@glmflash.hard45.CC.n\endcsname{45}
\expandafter\def\csname pn@glmflash.hard45.CC.pct\endcsname{49}
\expandafter\def\csname pn@glmflash.hard45.CC.seeds\endcsname{1}
\expandafter\def\csname pn@glmflash.hard45.CCvOC.b\endcsname{5}
\expandafter\def\csname pn@glmflash.hard45.CCvOC.c\endcsname{1}
\expandafter\def\csname pn@glmflash.hard45.CCvOC.diff\endcsname{+8.9}
\expandafter\def\csname pn@glmflash.hard45.CCvOC.hi\endcsname{+19.5}
\expandafter\def\csname pn@glmflash.hard45.CCvOC.lo\endcsname{-2.2}
\expandafter\def\csname pn@glmflash.hard45.CCvOC.n\endcsname{45}
\expandafter\def\csname pn@glmflash.hard45.CCvOC.p\endcsname{.22}
\expandafter\def\csname pn@glmflash.hard45.CCvmini.b\endcsname{4}
\expandafter\def\csname pn@glmflash.hard45.CCvmini.c\endcsname{2}
\expandafter\def\csname pn@glmflash.hard45.CCvmini.diff\endcsname{+4.4}
\expandafter\def\csname pn@glmflash.hard45.CCvmini.hi\endcsname{+15.3}
\expandafter\def\csname pn@glmflash.hard45.CCvmini.lo\endcsname{-6.7}
\expandafter\def\csname pn@glmflash.hard45.CCvmini.n\endcsname{45}
\expandafter\def\csname pn@glmflash.hard45.CCvmini.p\endcsname{.69}
\expandafter\def\csname pn@glmflash.hard45.OC.hi\endcsname{55}
\expandafter\def\csname pn@glmflash.hard45.OC.k\endcsname{18}
\expandafter\def\csname pn@glmflash.hard45.OC.lo\endcsname{27}
\expandafter\def\csname pn@glmflash.hard45.OC.n\endcsname{45}
\expandafter\def\csname pn@glmflash.hard45.OC.pct\endcsname{40}
\expandafter\def\csname pn@glmflash.hard45.OC.seeds\endcsname{1}
\expandafter\def\csname pn@glmflash.hard45.mini.hi\endcsname{59}
\expandafter\def\csname pn@glmflash.hard45.mini.k\endcsname{20}
\expandafter\def\csname pn@glmflash.hard45.mini.lo\endcsname{31}
\expandafter\def\csname pn@glmflash.hard45.mini.n\endcsname{45}
\expandafter\def\csname pn@glmflash.hard45.mini.pct\endcsname{44}
\expandafter\def\csname pn@glmflash.hard45.mini.seeds\endcsname{1}
\expandafter\def\csname pn@glmflash.hard45.minivOC.b\endcsname{4}
\expandafter\def\csname pn@glmflash.hard45.minivOC.c\endcsname{2}
\expandafter\def\csname pn@glmflash.hard45.minivOC.diff\endcsname{+4.4}
\expandafter\def\csname pn@glmflash.hard45.minivOC.hi\endcsname{+15.4}
\expandafter\def\csname pn@glmflash.hard45.minivOC.lo\endcsname{-6.7}
\expandafter\def\csname pn@glmflash.hard45.minivOC.n\endcsname{45}
\expandafter\def\csname pn@glmflash.hard45.minivOC.p\endcsname{.69}
\expandafter\def\csname pn@hy4.hard45.CC.hi\endcsname{65}
\expandafter\def\csname pn@hy4.hard45.CC.k\endcsname{23}
\expandafter\def\csname pn@hy4.hard45.CC.lo\endcsname{37}
\expandafter\def\csname pn@hy4.hard45.CC.n\endcsname{45}
\expandafter\def\csname pn@hy4.hard45.CC.pct\endcsname{51}
\expandafter\def\csname pn@hy4.hard45.CC.seeds\endcsname{1}
\expandafter\def\csname pn@hy4.hard45.CCvOC.b\endcsname{4}
\expandafter\def\csname pn@hy4.hard45.CCvOC.c\endcsname{2}
\expandafter\def\csname pn@hy4.hard45.CCvOC.diff\endcsname{+4.4}
\expandafter\def\csname pn@hy4.hard45.CCvOC.hi\endcsname{+15.3}
\expandafter\def\csname pn@hy4.hard45.CCvOC.lo\endcsname{-6.7}
\expandafter\def\csname pn@hy4.hard45.CCvOC.n\endcsname{45}
\expandafter\def\csname pn@hy4.hard45.CCvOC.p\endcsname{.69}
\expandafter\def\csname pn@hy4.hard45.CCvmini.b\endcsname{2}
\expandafter\def\csname pn@hy4.hard45.CCvmini.c\endcsname{5}
\expandafter\def\csname pn@hy4.hard45.CCvmini.diff\endcsname{-6.7}
\expandafter\def\csname pn@hy4.hard45.CCvmini.hi\endcsname{+5.2}
\expandafter\def\csname pn@hy4.hard45.CCvmini.lo\endcsname{-18.2}
\expandafter\def\csname pn@hy4.hard45.CCvmini.n\endcsname{45}
\expandafter\def\csname pn@hy4.hard45.CCvmini.p\endcsname{.45}
\expandafter\def\csname pn@hy4.hard45.OC.hi\endcsname{61}
\expandafter\def\csname pn@hy4.hard45.OC.k\endcsname{21}
\expandafter\def\csname pn@hy4.hard45.OC.lo\endcsname{33}
\expandafter\def\csname pn@hy4.hard45.OC.n\endcsname{45}
\expandafter\def\csname pn@hy4.hard45.OC.pct\endcsname{47}
\expandafter\def\csname pn@hy4.hard45.OC.seeds\endcsname{1}
\expandafter\def\csname pn@hy4.hard45.mini.hi\endcsname{71}
\expandafter\def\csname pn@hy4.hard45.mini.k\endcsname{26}
\expandafter\def\csname pn@hy4.hard45.mini.lo\endcsname{43}
\expandafter\def\csname pn@hy4.hard45.mini.n\endcsname{45}
\expandafter\def\csname pn@hy4.hard45.mini.pct\endcsname{58}
\expandafter\def\csname pn@hy4.hard45.mini.seeds\endcsname{1}
\expandafter\def\csname pn@hy4.hard45.minivOC.b\endcsname{6}
\expandafter\def\csname pn@hy4.hard45.minivOC.c\endcsname{1}
\expandafter\def\csname pn@hy4.hard45.minivOC.diff\endcsname{+11.1}
\expandafter\def\csname pn@hy4.hard45.minivOC.hi\endcsname{+22.2}
\expandafter\def\csname pn@hy4.hard45.minivOC.lo\endcsname{-0.7}
\expandafter\def\csname pn@hy4.hard45.minivOC.n\endcsname{45}
\expandafter\def\csname pn@hy4.hard45.minivOC.p\endcsname{.12}
\expandafter\def\csname pn@mde.hard45.disc\endcsname{14}
\expandafter\def\csname pn@mde.hard45.nmin80\endcsname{55}
\expandafter\def\csname pn@mde.hard45.powermax\endcsname{62}
\expandafter\def\csname pn@mde.hard45.pp\endcsname{13}
\expandafter\def\csname pn@mde.hard45.pp50\endcsname{12.9}
\expandafter\def\csname pn@mde.hard45.ppexact\endcsname{--}
\expandafter\def\csname pn@mde.pool447.disc\endcsname{14}
\expandafter\def\csname pn@mde.pool447.nmin80\endcsname{54}
\expandafter\def\csname pn@mde.pool447.powermax\endcsname{100}
\expandafter\def\csname pn@mde.pool447.pp\endcsname{5}
\expandafter\def\csname pn@mde.pool447.pp50\endcsname{3.7}
\expandafter\def\csname pn@mde.pool447.ppexact\endcsname{5.2}
\expandafter\def\csname pn@opus.hard45.CC.hi\endcsname{89}
\expandafter\def\csname pn@opus.hard45.CC.k\endcsname{36}
\expandafter\def\csname pn@opus.hard45.CC.lo\endcsname{66}
\expandafter\def\csname pn@opus.hard45.CC.n\endcsname{45}
\expandafter\def\csname pn@opus.hard45.CC.pct\endcsname{80}
\expandafter\def\csname pn@opus.hard45.CC.seeds\endcsname{3}
\expandafter\def\csname pn@out.dsflash.hard45.CC.fail\endcsname{24}
\expandafter\def\csname pn@out.dsflash.hard45.CC.pass\endcsname{21}
\expandafter\def\csname pn@out.dsflash.hard45.OC.cap\endcsname{1}
\expandafter\def\csname pn@out.dsflash.hard45.OC.fail\endcsname{25}
\expandafter\def\csname pn@out.dsflash.hard45.OC.pass\endcsname{19}
\expandafter\def\csname pn@out.dsflash.hard45.dsh.cap\endcsname{3}
\expandafter\def\csname pn@out.dsflash.hard45.dsh.fail\endcsname{21}
\expandafter\def\csname pn@out.dsflash.hard45.dsh.pass\endcsname{21}
\expandafter\def\csname pn@out.dsflash.hard45.mini.fail\endcsname{23}
\expandafter\def\csname pn@out.dsflash.hard45.mini.pass\endcsname{22}
\expandafter\def\csname pn@out.glmflash.hard45.CC.cap\endcsname{1}
\expandafter\def\csname pn@out.glmflash.hard45.CC.fail\endcsname{22}
\expandafter\def\csname pn@out.glmflash.hard45.CC.pass\endcsname{22}
\expandafter\def\csname pn@out.glmflash.hard45.OC.fail\endcsname{27}
\expandafter\def\csname pn@out.glmflash.hard45.OC.pass\endcsname{18}
\expandafter\def\csname pn@out.glmflash.hard45.mini.fail\endcsname{25}
\expandafter\def\csname pn@out.glmflash.hard45.mini.pass\endcsname{20}
\expandafter\def\csname pn@out.hy4.hard45.CC.fail\endcsname{22}
\expandafter\def\csname pn@out.hy4.hard45.CC.pass\endcsname{23}
\expandafter\def\csname pn@out.hy4.hard45.OC.fail\endcsname{24}
\expandafter\def\csname pn@out.hy4.hard45.OC.pass\endcsname{21}
\expandafter\def\csname pn@out.hy4.hard45.mini.fail\endcsname{19}
\expandafter\def\csname pn@out.hy4.hard45.mini.pass\endcsname{26}
\expandafter\def\csname pn@out.opus.hard45.CC.fail\endcsname{9}
\expandafter\def\csname pn@out.opus.hard45.CC.pass\endcsname{36}
\expandafter\def\csname pn@out.qwen36.hard45.CC.cap\endcsname{1}
\expandafter\def\csname pn@out.qwen36.hard45.CC.fail\endcsname{33}
\expandafter\def\csname pn@out.qwen36.hard45.CC.pass\endcsname{11}
\expandafter\def\csname pn@out.qwen36.hard45.OC.fail\endcsname{34}
\expandafter\def\csname pn@out.qwen36.hard45.OC.pass\endcsname{11}
\expandafter\def\csname pn@out.qwen36.hard45.mini.fail\endcsname{28}
\expandafter\def\csname pn@out.qwen36.hard45.mini.overflow\endcsname{2}
\expandafter\def\csname pn@out.qwen36.hard45.mini.pass\endcsname{15}
\expandafter\def\csname pn@out.qwen36.pool447.CC.cap\endcsname{2}
\expandafter\def\csname pn@out.qwen36.pool447.CC.fail\endcsname{133}
\expandafter\def\csname pn@out.qwen36.pool447.CC.pass\endcsname{310}
\expandafter\def\csname pn@out.qwen36.pool447.CC.void\endcsname{2}
\expandafter\def\csname pn@out.qwen36.pool447.OC.fail\endcsname{149}
\expandafter\def\csname pn@out.qwen36.pool447.OC.pass\endcsname{297}
\expandafter\def\csname pn@out.qwen36.pool447.OC.void\endcsname{1}
\expandafter\def\csname pn@out.qwen36.pool447.mini.fail\endcsname{121}
\expandafter\def\csname pn@out.qwen36.pool447.mini.overflow\endcsname{6}
\expandafter\def\csname pn@out.qwen36.pool447.mini.pass\endcsname{318}
\expandafter\def\csname pn@out.qwen36.pool447.mini.void\endcsname{2}
\expandafter\def\csname pn@out.qwen38.hard45.CC.fail\endcsname{23}
\expandafter\def\csname pn@out.qwen38.hard45.CC.overflow\endcsname{1}
\expandafter\def\csname pn@out.qwen38.hard45.CC.pass\endcsname{19}
\expandafter\def\csname pn@out.qwen38.hard45.CC.void\endcsname{2}
\expandafter\def\csname pn@out.qwen38.hard45.OC.cap\endcsname{6}
\expandafter\def\csname pn@out.qwen38.hard45.OC.fail\endcsname{22}
\expandafter\def\csname pn@out.qwen38.hard45.OC.pass\endcsname{17}
\expandafter\def\csname pn@out.qwen38.hard45.mini.fail\endcsname{17}
\expandafter\def\csname pn@out.qwen38.hard45.mini.overflow\endcsname{11}
\expandafter\def\csname pn@out.qwen38.hard45.mini.pass\endcsname{17}
\expandafter\def\csname pn@out.qwen38.pool447.CC.cap\endcsname{1}
\expandafter\def\csname pn@out.qwen38.pool447.CC.fail\endcsname{95}
\expandafter\def\csname pn@out.qwen38.pool447.CC.overflow\endcsname{1}
\expandafter\def\csname pn@out.qwen38.pool447.CC.pass\endcsname{347}
\expandafter\def\csname pn@out.qwen38.pool447.CC.void\endcsname{3}
\expandafter\def\csname pn@out.qwen38.pool447.OC.cutoff\endcsname{33}
\expandafter\def\csname pn@out.qwen38.pool447.OC.fail\endcsname{100}
\expandafter\def\csname pn@out.qwen38.pool447.OC.pass\endcsname{312}
\expandafter\def\csname pn@out.qwen38.pool447.OC.void\endcsname{2}
\expandafter\def\csname pn@out.qwen38.pool447.mini.cap\endcsname{3}
\expandafter\def\csname pn@out.qwen38.pool447.mini.fail\endcsname{71}
\expandafter\def\csname pn@out.qwen38.pool447.mini.overflow\endcsname{18}
\expandafter\def\csname pn@out.qwen38.pool447.mini.pass\endcsname{353}
\expandafter\def\csname pn@out.qwen38.pool447.mini.void\endcsname{2}
\expandafter\def\csname pn@price.dsflash.hit\endcsname{0.05}
\expandafter\def\csname pn@price.dsflash.miss\endcsname{1.5}
\expandafter\def\csname pn@price.dsflash.out\endcsname{4.5}
\expandafter\def\csname pn@price.dsflash.ratio\endcsname{0.033}
\expandafter\def\csname pn@price.glmflash.hit\endcsname{0.23}
\expandafter\def\csname pn@price.glmflash.miss\endcsname{0.8}
\expandafter\def\csname pn@price.glmflash.out\endcsname{2.8}
\expandafter\def\csname pn@price.glmflash.ratio\endcsname{0.287}
\expandafter\def\csname pn@price.hy4.hit\endcsname{0.3}
\expandafter\def\csname pn@price.hy4.miss\endcsname{6.0}
\expandafter\def\csname pn@price.hy4.out\endcsname{18.0}
\expandafter\def\csname pn@price.hy4.ratio\endcsname{0.050}
\expandafter\def\csname pn@qwen36.hard45.CC.hi\endcsname{39}
\expandafter\def\csname pn@qwen36.hard45.CC.k\endcsname{11}
\expandafter\def\csname pn@qwen36.hard45.CC.lo\endcsname{14}
\expandafter\def\csname pn@qwen36.hard45.CC.n\endcsname{45}
\expandafter\def\csname pn@qwen36.hard45.CC.pct\endcsname{24}
\expandafter\def\csname pn@qwen36.hard45.CC.seeds\endcsname{2}
\expandafter\def\csname pn@qwen36.hard45.CCvOC.b\endcsname{3}
\expandafter\def\csname pn@qwen36.hard45.CCvOC.c\endcsname{3}
\expandafter\def\csname pn@qwen36.hard45.CCvOC.diff\endcsname{+0.0}
\expandafter\def\csname pn@qwen36.hard45.CCvOC.hi\endcsname{+11.8}
\expandafter\def\csname pn@qwen36.hard45.CCvOC.lo\endcsname{-11.8}
\expandafter\def\csname pn@qwen36.hard45.CCvOC.n\endcsname{45}
\expandafter\def\csname pn@qwen36.hard45.CCvOC.p\endcsname{1.00}
\expandafter\def\csname pn@qwen36.hard45.CCvmini.b\endcsname{4}
\expandafter\def\csname pn@qwen36.hard45.CCvmini.c\endcsname{8}
\expandafter\def\csname pn@qwen36.hard45.CCvmini.diff\endcsname{-8.9}
\expandafter\def\csname pn@qwen36.hard45.CCvmini.hi\endcsname{+6.6}
\expandafter\def\csname pn@qwen36.hard45.CCvmini.lo\endcsname{-23.9}
\expandafter\def\csname pn@qwen36.hard45.CCvmini.n\endcsname{45}
\expandafter\def\csname pn@qwen36.hard45.CCvmini.p\endcsname{.39}
\expandafter\def\csname pn@qwen36.hard45.OC.hi\endcsname{39}
\expandafter\def\csname pn@qwen36.hard45.OC.k\endcsname{11}
\expandafter\def\csname pn@qwen36.hard45.OC.lo\endcsname{14}
\expandafter\def\csname pn@qwen36.hard45.OC.n\endcsname{45}
\expandafter\def\csname pn@qwen36.hard45.OC.pct\endcsname{24}
\expandafter\def\csname pn@qwen36.hard45.OC.seeds\endcsname{2}
\expandafter\def\csname pn@qwen36.hard45.mini.hi\endcsname{48}
\expandafter\def\csname pn@qwen36.hard45.mini.k\endcsname{15}
\expandafter\def\csname pn@qwen36.hard45.mini.lo\endcsname{21}
\expandafter\def\csname pn@qwen36.hard45.mini.n\endcsname{45}
\expandafter\def\csname pn@qwen36.hard45.mini.pct\endcsname{33}
\expandafter\def\csname pn@qwen36.hard45.mini.seeds\endcsname{2}
\expandafter\def\csname pn@qwen36.hard45.minivOC.b\endcsname{6}
\expandafter\def\csname pn@qwen36.hard45.minivOC.c\endcsname{2}
\expandafter\def\csname pn@qwen36.hard45.minivOC.diff\endcsname{+8.9}
\expandafter\def\csname pn@qwen36.hard45.minivOC.hi\endcsname{+21.5}
\expandafter\def\csname pn@qwen36.hard45.minivOC.lo\endcsname{-4.0}
\expandafter\def\csname pn@qwen36.hard45.minivOC.n\endcsname{45}
\expandafter\def\csname pn@qwen36.hard45.minivOC.p\endcsname{.29}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.b\endcsname{43}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.c\endcsname{30}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.diff\endcsname{+2.9}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.hi\endcsname{+6.7}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.hinine\endcsname{+6.1}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.lo\endcsname{-0.9}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.lonine\endcsname{-0.3}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.n\endcsname{445}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.p\endcsname{.16}
\expandafter\def\csname pn@qwen36.pool447.CCvOC.tost\endcsname{no}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.b\endcsname{26}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.c\endcsname{34}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.diff\endcsname{-1.8}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.hi\endcsname{+1.6}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.hinine\endcsname{+1.1}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.lo\endcsname{-5.2}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.lonine\endcsname{-4.7}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.n\endcsname{445}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.p\endcsname{.37}
\expandafter\def\csname pn@qwen36.pool447.CCvmini.tost\endcsname{yes}
\expandafter\def\csname pn@qwen36.pool447.minivOC.b\endcsname{45}
\expandafter\def\csname pn@qwen36.pool447.minivOC.c\endcsname{24}
\expandafter\def\csname pn@qwen36.pool447.minivOC.diff\endcsname{+4.7}
\expandafter\def\csname pn@qwen36.pool447.minivOC.hi\endcsname{+8.4}
\expandafter\def\csname pn@qwen36.pool447.minivOC.hinine\endcsname{+7.8}
\expandafter\def\csname pn@qwen36.pool447.minivOC.lo\endcsname{+1.1}
\expandafter\def\csname pn@qwen36.pool447.minivOC.lonine\endcsname{+1.6}
\expandafter\def\csname pn@qwen36.pool447.minivOC.n\endcsname{445}
\expandafter\def\csname pn@qwen36.pool447.minivOC.p\endcsname{.02}
\expandafter\def\csname pn@qwen36.pool447.minivOC.tost\endcsname{no}
\expandafter\def\csname pn@qwen38.hard45.CC.hi\endcsname{59}
\expandafter\def\csname pn@qwen38.hard45.CC.k\endcsname{19}
\expandafter\def\csname pn@qwen38.hard45.CC.lo\endcsname{30}
\expandafter\def\csname pn@qwen38.hard45.CC.n\endcsname{43}
\expandafter\def\csname pn@qwen38.hard45.CC.pct\endcsname{44}
\expandafter\def\csname pn@qwen38.hard45.CC.seeds\endcsname{2}
\expandafter\def\csname pn@qwen38.hard45.CCvOC.b\endcsname{3}
\expandafter\def\csname pn@qwen38.hard45.CCvOC.c\endcsname{0}
\expandafter\def\csname pn@qwen38.hard45.CCvOC.diff\endcsname{+7.0}
\expandafter\def\csname pn@qwen38.hard45.CCvOC.hi\endcsname{+15.5}
\expandafter\def\csname pn@qwen38.hard45.CCvOC.lo\endcsname{-1.8}
\expandafter\def\csname pn@qwen38.hard45.CCvOC.n\endcsname{43}
\expandafter\def\csname pn@qwen38.hard45.CCvOC.p\endcsname{.25}
\expandafter\def\csname pn@qwen38.hard45.CCvmini.b\endcsname{5}
\expandafter\def\csname pn@qwen38.hard45.CCvmini.c\endcsname{2}
\expandafter\def\csname pn@qwen38.hard45.CCvmini.diff\endcsname{+7.0}
\expandafter\def\csname pn@qwen38.hard45.CCvmini.hi\endcsname{+19.1}
\expandafter\def\csname pn@qwen38.hard45.CCvmini.lo\endcsname{-5.5}
\expandafter\def\csname pn@qwen38.hard45.CCvmini.n\endcsname{43}
\expandafter\def\csname pn@qwen38.hard45.CCvmini.p\endcsname{.45}
\expandafter\def\csname pn@qwen38.hard45.OC.hi\endcsname{52}
\expandafter\def\csname pn@qwen38.hard45.OC.k\endcsname{17}
\expandafter\def\csname pn@qwen38.hard45.OC.lo\endcsname{25}
\expandafter\def\csname pn@qwen38.hard45.OC.n\endcsname{45}
\expandafter\def\csname pn@qwen38.hard45.OC.pct\endcsname{38}
\expandafter\def\csname pn@qwen38.hard45.OC.seeds\endcsname{2}
\expandafter\def\csname pn@qwen38.hard45.mini.hi\endcsname{52}
\expandafter\def\csname pn@qwen38.hard45.mini.k\endcsname{17}
\expandafter\def\csname pn@qwen38.hard45.mini.lo\endcsname{25}
\expandafter\def\csname pn@qwen38.hard45.mini.n\endcsname{45}
\expandafter\def\csname pn@qwen38.hard45.mini.pct\endcsname{38}
\expandafter\def\csname pn@qwen38.hard45.mini.seeds\endcsname{2}
\expandafter\def\csname pn@qwen38.hard45.minivOC.b\endcsname{3}
\expandafter\def\csname pn@qwen38.hard45.minivOC.c\endcsname{3}
\expandafter\def\csname pn@qwen38.hard45.minivOC.diff\endcsname{+0.0}
\expandafter\def\csname pn@qwen38.hard45.minivOC.hi\endcsname{+11.2}
\expandafter\def\csname pn@qwen38.hard45.minivOC.lo\endcsname{-11.2}
\expandafter\def\csname pn@qwen38.hard45.minivOC.n\endcsname{45}
\expandafter\def\csname pn@qwen38.hard45.minivOC.p\endcsname{1.00}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.b\endcsname{52}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.c\endcsname{17}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.diff\endcsname{+7.9}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.hi\endcsname{+11.5}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.hinine\endcsname{+10.9}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.lo\endcsname{+4.3}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.lonine\endcsname{+4.8}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.n\endcsname{444}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.p\endcsname{$<$.001}
\expandafter\def\csname pn@qwen38.pool447.CCvOC.tost\endcsname{no}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.b\endcsname{17}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.c\endcsname{23}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.diff\endcsname{-1.4}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.hi\endcsname{+1.5}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.hinine\endcsname{+1.0}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.lo\endcsname{-4.2}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.lonine\endcsname{-3.7}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.n\endcsname{444}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.p\endcsname{.43}
\expandafter\def\csname pn@qwen38.pool447.CCvmini.tost\endcsname{yes}
\expandafter\def\csname pn@qwen38.pool447.minivOC.b\endcsname{57}
\expandafter\def\csname pn@qwen38.pool447.minivOC.c\endcsname{16}
\expandafter\def\csname pn@qwen38.pool447.minivOC.diff\endcsname{+9.2}
\expandafter\def\csname pn@qwen38.pool447.minivOC.hi\endcsname{+12.9}
\expandafter\def\csname pn@qwen38.pool447.minivOC.hinine\endcsname{+12.3}
\expandafter\def\csname pn@qwen38.pool447.minivOC.lo\endcsname{+5.5}
\expandafter\def\csname pn@qwen38.pool447.minivOC.lonine\endcsname{+6.1}
\expandafter\def\csname pn@qwen38.pool447.minivOC.n\endcsname{445}
\expandafter\def\csname pn@qwen38.pool447.minivOC.p\endcsname{$<$.001}
\expandafter\def\csname pn@qwen38.pool447.minivOC.tost\endcsname{no}
\expandafter\def\csname pn@reprice.dsflash.ds.CC.cny\endcsname{0.98}
\expandafter\def\csname pn@reprice.dsflash.ds.CCvOC\endcsname{1.47}
\expandafter\def\csname pn@reprice.dsflash.ds.CCvmini\endcsname{0.95}
\expandafter\def\csname pn@reprice.dsflash.ds.OC.cny\endcsname{0.66}
\expandafter\def\csname pn@reprice.dsflash.ds.mini.cny\endcsname{1.02}
\expandafter\def\csname pn@reprice.dsflash.zhipu.CC.cny\endcsname{2.29}
\expandafter\def\csname pn@reprice.dsflash.zhipu.CCvOC\endcsname{1.42}
\expandafter\def\csname pn@reprice.dsflash.zhipu.CCvmini\endcsname{0.79}
\expandafter\def\csname pn@reprice.dsflash.zhipu.OC.cny\endcsname{1.61}
\expandafter\def\csname pn@reprice.dsflash.zhipu.mini.cny\endcsname{2.89}
\expandafter\def\csname pn@reprice.glmflash.ds.CC.cny\endcsname{0.88}
\expandafter\def\csname pn@reprice.glmflash.ds.CCvOC\endcsname{2.76}
\expandafter\def\csname pn@reprice.glmflash.ds.CCvmini\endcsname{2.09}
\expandafter\def\csname pn@reprice.glmflash.ds.OC.cny\endcsname{0.32}
\expandafter\def\csname pn@reprice.glmflash.ds.mini.cny\endcsname{0.42}
\expandafter\def\csname pn@reprice.glmflash.zhipu.CC.cny\endcsname{1.81}
\expandafter\def\csname pn@reprice.glmflash.zhipu.CCvOC\endcsname{3.22}
\expandafter\def\csname pn@reprice.glmflash.zhipu.CCvmini\endcsname{1.86}
\expandafter\def\csname pn@reprice.glmflash.zhipu.OC.cny\endcsname{0.56}
\expandafter\def\csname pn@reprice.glmflash.zhipu.mini.cny\endcsname{0.97}
\expandafter\def\csname pn@reprice.hy4.ds.CC.cny\endcsname{0.59}
\expandafter\def\csname pn@reprice.hy4.ds.CCvOC\endcsname{1.14}
\expandafter\def\csname pn@reprice.hy4.ds.CCvmini\endcsname{0.67}
\expandafter\def\csname pn@reprice.hy4.ds.OC.cny\endcsname{0.52}
\expandafter\def\csname pn@reprice.hy4.ds.mini.cny\endcsname{0.87}
\expandafter\def\csname pn@reprice.hy4.zhipu.CC.cny\endcsname{1.34}
\expandafter\def\csname pn@reprice.hy4.zhipu.CCvOC\endcsname{1.36}
\expandafter\def\csname pn@reprice.hy4.zhipu.CCvmini\endcsname{0.75}
\expandafter\def\csname pn@reprice.hy4.zhipu.OC.cny\endcsname{0.99}
\expandafter\def\csname pn@reprice.hy4.zhipu.mini.cny\endcsname{1.78}
\expandafter\def\csname pn@steps.dsflash.hard45.CC.mean\endcsname{103.6}
\expandafter\def\csname pn@steps.dsflash.hard45.CC.median\endcsname{93}
\expandafter\def\csname pn@steps.dsflash.hard45.OC.mean\endcsname{88.2}
\expandafter\def\csname pn@steps.dsflash.hard45.OC.median\endcsname{89}
\expandafter\def\csname pn@steps.dsflash.hard45.dsh.mean\endcsname{111.2}
\expandafter\def\csname pn@steps.dsflash.hard45.dsh.median\endcsname{102}
\expandafter\def\csname pn@steps.dsflash.hard45.mini.mean\endcsname{141.1}
\expandafter\def\csname pn@steps.dsflash.hard45.mini.median\endcsname{137}
\expandafter\def\csname pn@steps.glmflash.hard45.CC.mean\endcsname{88.1}
\expandafter\def\csname pn@steps.glmflash.hard45.CC.median\endcsname{78}
\expandafter\def\csname pn@steps.glmflash.hard45.OC.mean\endcsname{55.0}
\expandafter\def\csname pn@steps.glmflash.hard45.OC.median\endcsname{51}
\expandafter\def\csname pn@steps.glmflash.hard45.mini.mean\endcsname{80.2}
\expandafter\def\csname pn@steps.glmflash.hard45.mini.median\endcsname{70}
\expandafter\def\csname pn@steps.hy4.hard45.CC.mean\endcsname{79.9}
\expandafter\def\csname pn@steps.hy4.hard45.CC.median\endcsname{74}
\expandafter\def\csname pn@steps.hy4.hard45.OC.mean\endcsname{66.8}
\expandafter\def\csname pn@steps.hy4.hard45.OC.median\endcsname{53}
\expandafter\def\csname pn@steps.hy4.hard45.mini.mean\endcsname{87.8}
\expandafter\def\csname pn@steps.hy4.hard45.mini.median\endcsname{86}
\expandafter\def\csname pn@steps.opus.hard45.CC.mean\endcsname{40.0}
\expandafter\def\csname pn@steps.opus.hard45.CC.median\endcsname{33}
\expandafter\def\csname pn@steps.qwen36.hard45.CC.mean\endcsname{107.3}
\expandafter\def\csname pn@steps.qwen36.hard45.CC.median\endcsname{101}
\expandafter\def\csname pn@steps.qwen36.hard45.OC.mean\endcsname{54.9}
\expandafter\def\csname pn@steps.qwen36.hard45.OC.median\endcsname{43}
\expandafter\def\csname pn@steps.qwen36.hard45.mini.mean\endcsname{118.5}
\expandafter\def\csname pn@steps.qwen36.hard45.mini.median\endcsname{107}
\expandafter\def\csname pn@steps.qwen36.pool447.CC.mean\endcsname{64.8}
\expandafter\def\csname pn@steps.qwen36.pool447.CC.median\endcsname{55}
\expandafter\def\csname pn@steps.qwen36.pool447.OC.mean\endcsname{36.7}
\expandafter\def\csname pn@steps.qwen36.pool447.OC.median\endcsname{28}
\expandafter\def\csname pn@steps.qwen36.pool447.mini.mean\endcsname{77.8}
\expandafter\def\csname pn@steps.qwen36.pool447.mini.median\endcsname{71}
\expandafter\def\csname pn@steps.qwen38.hard45.CC.mean\endcsname{87.1}
\expandafter\def\csname pn@steps.qwen38.hard45.CC.median\endcsname{70}
\expandafter\def\csname pn@steps.qwen38.hard45.OC.mean\endcsname{75.4}
\expandafter\def\csname pn@steps.qwen38.hard45.OC.median\endcsname{71}
\expandafter\def\csname pn@steps.qwen38.hard45.mini.mean\endcsname{74.0}
\expandafter\def\csname pn@steps.qwen38.hard45.mini.median\endcsname{73}
\expandafter\def\csname pn@steps.qwen38.pool447.CC.mean\endcsname{54.3}
\expandafter\def\csname pn@steps.qwen38.pool447.CC.median\endcsname{50}
\expandafter\def\csname pn@steps.qwen38.pool447.OC.mean\endcsname{47.8}
\expandafter\def\csname pn@steps.qwen38.pool447.OC.median\endcsname{42}
\expandafter\def\csname pn@steps.qwen38.pool447.mini.mean\endcsname{57.4}
\expandafter\def\csname pn@steps.qwen38.pool447.mini.median\endcsname{53}
\makeatother


==> numbers_a4.tex <==
\makeatletter
\DeclareRobustCommand{\pn}[1]{\csname pn@#1\endcsname}
\expandafter\def\csname pn@budget.cc.args.run\endcsname{11{,}719}
\expandafter\def\csname pn@budget.cc.compact\endcsname{8}
\expandafter\def\csname pn@budget.cc.compact.pre.k\endcsname{168}
\expandafter\def\csname pn@budget.cc.cpt\endcsname{3.84}
\expandafter\def\csname pn@budget.cc.fixed\endcsname{17{,}134}
\expandafter\def\csname pn@budget.cc.fixed.harness\endcsname{16{,}581}
\expandafter\def\csname pn@budget.cc.job\endcsname{\texttt{cc-\allowbreak glm53f-\allowbreak hard45-\allowbreak nw}}
\expandafter\def\csname pn@budget.cc.obs.mean\endcsname{1{,}237}
\expandafter\def\csname pn@budget.cc.obs.median\endcsname{392}
\expandafter\def\csname pn@budget.cc.obs.n\endcsname{4{,}403}
\expandafter\def\csname pn@budget.cc.obs.p90\endcsname{3{,}095}
\expandafter\def\csname pn@budget.cc.obs.run\endcsname{31{,}557}
\expandafter\def\csname pn@budget.cc.obs.top\endcsname{Bash}
\expandafter\def\csname pn@budget.cc.obs.toppct\endcsname{68}
\expandafter\def\csname pn@budget.cc.obs.totalM\endcsname{5.4}
\expandafter\def\csname pn@budget.cc.perstep.gap\endcsname{+6\%}
\expandafter\def\csname pn@budget.cc.perstep.measured\endcsname{75{,}286}
\expandafter\def\csname pn@budget.cc.perstep.measured.k\endcsname{75.3}
\expandafter\def\csname pn@budget.cc.perstep.recon\endcsname{80{,}060}
\expandafter\def\csname pn@budget.cc.perstep.recon.k\endcsname{80.1}
\expandafter\def\csname pn@budget.cc.steps\endcsname{88.1}
\expandafter\def\csname pn@budget.cc.text.run\endcsname{58{,}359}
\expandafter\def\csname pn@budget.cc.trials\endcsname{45}
\expandafter\def\csname pn@budget.issue.chars\endcsname{2{,}049}
\expandafter\def\csname pn@budget.issue.tok\endcsname{554}
\expandafter\def\csname pn@budget.mini.args.run\endcsname{14{,}554}
\expandafter\def\csname pn@budget.mini.compact\endcsname{0}
\expandafter\def\csname pn@budget.mini.cpt\endcsname{2.22}
\expandafter\def\csname pn@budget.mini.fixed\endcsname{1{,}382}
\expandafter\def\csname pn@budget.mini.fixed.harness\endcsname{829}
\expandafter\def\csname pn@budget.mini.job\endcsname{\texttt{mini-\allowbreak glm53f-\allowbreak hard45b-\allowbreak nw}}
\expandafter\def\csname pn@budget.mini.obs.mean\endcsname{1{,}186}
\expandafter\def\csname pn@budget.mini.obs.median\endcsname{461}
\expandafter\def\csname pn@budget.mini.obs.n\endcsname{3{,}787}
\expandafter\def\csname pn@budget.mini.obs.p90\endcsname{3{,}121}
\expandafter\def\csname pn@budget.mini.obs.run\endcsname{44{,}871}
\expandafter\def\csname pn@budget.mini.obs.top\endcsname{bash}
\expandafter\def\csname pn@budget.mini.obs.toppct\endcsname{100}
\expandafter\def\csname pn@budget.mini.obs.totalM\endcsname{4.5}
\expandafter\def\csname pn@budget.mini.perstep.gap\endcsname{$-$13\%}
\expandafter\def\csname pn@budget.mini.perstep.measured\endcsname{45{,}897}
\expandafter\def\csname pn@budget.mini.perstep.measured.k\endcsname{45.9}
\expandafter\def\csname pn@budget.mini.perstep.recon\endcsname{39{,}933}
\expandafter\def\csname pn@budget.mini.perstep.recon.k\endcsname{39.9}
\expandafter\def\csname pn@budget.mini.steps\endcsname{80.2}
\expandafter\def\csname pn@budget.mini.template.chars\endcsname{2{,}860}
\expandafter\def\csname pn@budget.mini.text.run\endcsname{1{,}715}
\expandafter\def\csname pn@budget.mini.trials\endcsname{45}
\expandafter\def\csname pn@budget.obs.spread\endcsname{1.12}
\expandafter\def\csname pn@budget.oc.args.run\endcsname{5{,}130}
\expandafter\def\csname pn@budget.oc.compact\endcsname{0}
\expandafter\def\csname pn@budget.oc.compact.limit.k\endcsname{78}
\expandafter\def\csname pn@budget.oc.cpt\endcsname{3.85}
\expandafter\def\csname pn@budget.oc.fixed\endcsname{7{,}579}
\expandafter\def\csname pn@budget.oc.fixed.harness\endcsname{7{,}025}
\expandafter\def\csname pn@budget.oc.job\endcsname{\texttt{oc-\allowbreak glm53f-\allowbreak hard45-\allowbreak nw-\allowbreak rg}}
\expandafter\def\csname pn@budget.oc.obs.mean\endcsname{1{,}103}
\expandafter\def\csname pn@budget.oc.obs.median\endcsname{311}
\expandafter\def\csname pn@budget.oc.obs.n\endcsname{2{,}633}
\expandafter\def\csname pn@budget.oc.obs.p90\endcsname{3{,}049}
\expandafter\def\csname pn@budget.oc.obs.run\endcsname{16{,}781}
\expandafter\def\csname pn@budget.oc.obs.top\endcsname{read}
\expandafter\def\csname pn@budget.oc.obs.toppct\endcsname{49}
\expandafter\def\csname pn@budget.oc.obs.totalM\endcsname{2.9}
\expandafter\def\csname pn@budget.oc.perstep.gap\endcsname{$-$6\%}
\expandafter\def\csname pn@budget.oc.perstep.measured\endcsname{35{,}039}
\expandafter\def\csname pn@budget.oc.perstep.measured.k\endcsname{35.0}
\expandafter\def\csname pn@budget.oc.perstep.recon\endcsname{33{,}068}
\expandafter\def\csname pn@budget.oc.perstep.recon.k\endcsname{33.1}
\expandafter\def\csname pn@budget.oc.steps\endcsname{55.1}
\expandafter\def\csname pn@budget.oc.text.run\endcsname{21{,}900}
\expandafter\def\csname pn@budget.oc.trials\endcsname{45}
\expandafter\def\csname pn@budget.ratio.ccvsmin\endcsname{2.1}
\makeatother


==> numbers_a67.tex <==
\makeatletter
\@ifundefined{pn}{\DeclareRobustCommand{\pn}[1]{\csname pn@#1\endcsname}}{}
\expandafter\def\csname pn@opus.bashonly.k1\endcsname{36}
\expandafter\def\csname pn@opus.bashonly.k2\endcsname{37}
\expandafter\def\csname pn@opus.bashonly1.ci\endcsname{[66.2, 89.1]}
\expandafter\def\csname pn@opus.bashonly1.cihi\endcsname{89.1}
\expandafter\def\csname pn@opus.bashonly1.cilo\endcsname{66.2}
\expandafter\def\csname pn@opus.bashonly1.cost\endcsname{1.42}
\expandafter\def\csname pn@opus.bashonly1.costmed\endcsname{1.18}
\expandafter\def\csname pn@opus.bashonly1.costsum\endcsname{63.7}
\expandafter\def\csname pn@opus.bashonly1.flippct\endcsname{11.9}
\expandafter\def\csname pn@opus.bashonly1.flips\endcsname{16/135}
\expandafter\def\csname pn@opus.bashonly1.job\endcsname{\texttt{cc-\allowbreak opus-\allowbreak hard45-\allowbreak nw-\allowbreak c2}}
\expandafter\def\csname pn@opus.bashonly1.k\endcsname{36}
\expandafter\def\csname pn@opus.bashonly1.mcnemar\endcsname{1.00}
\expandafter\def\csname pn@opus.bashonly1.n\endcsname{45}
\expandafter\def\csname pn@opus.bashonly1.out\endcsname{13{,}539}
\expandafter\def\csname pn@opus.bashonly1.pct\endcsname{80.0}
\expandafter\def\csname pn@opus.bashonly1.reas\endcsname{5{,}378}
\expandafter\def\csname pn@opus.bashonly1.rows\endcsname{45}
\expandafter\def\csname pn@opus.bashonly1.steps\endcsname{31}
\expandafter\def\csname pn@opus.bashonly1.version\endcsname{2.1.263}
\expandafter\def\csname pn@opus.bashonly2.ci\endcsname{[68.7, 90.7]}
\expandafter\def\csname pn@opus.bashonly2.cihi\endcsname{90.7}
\expandafter\def\csname pn@opus.bashonly2.cilo\endcsname{68.7}
\expandafter\def\csname pn@opus.bashonly2.cost\endcsname{1.63}
\expandafter\def\csname pn@opus.bashonly2.costmed\endcsname{1.05}
\expandafter\def\csname pn@opus.bashonly2.costsum\endcsname{73.6}
\expandafter\def\csname pn@opus.bashonly2.flippct\endcsname{5.2}
\expandafter\def\csname pn@opus.bashonly2.flips\endcsname{7/135}
\expandafter\def\csname pn@opus.bashonly2.job\endcsname{\texttt{cc-\allowbreak opus-\allowbreak hard45-\allowbreak nw-\allowbreak c2-\allowbreak s2}}
\expandafter\def\csname pn@opus.bashonly2.k\endcsname{37}
\expandafter\def\csname pn@opus.bashonly2.mcnemar\endcsname{1.00}
\expandafter\def\csname pn@opus.bashonly2.n\endcsname{45}
\expandafter\def\csname pn@opus.bashonly2.out\endcsname{12{,}250}
\expandafter\def\csname pn@opus.bashonly2.pct\endcsname{82.2}
\expandafter\def\csname pn@opus.bashonly2.reas\endcsname{5{,}853}
\expandafter\def\csname pn@opus.bashonly2.rows\endcsname{45}
\expandafter\def\csname pn@opus.bashonly2.steps\endcsname{28}
\expandafter\def\csname pn@opus.bashonly2.version\endcsname{2.1.263}
\expandafter\def\csname pn@opus.ctrl.cost\endcsname{1.65}
\expandafter\def\csname pn@opus.ctrl.costmed\endcsname{1.39}
\expandafter\def\csname pn@opus.ctrl.floor\endcsname{6/135}
\expandafter\def\csname pn@opus.ctrl.floorpct\endcsname{4.4}
\expandafter\def\csname pn@opus.ctrl.k1\endcsname{36}
\expandafter\def\csname pn@opus.ctrl.k2\endcsname{35}
\expandafter\def\csname pn@opus.ctrl.k3\endcsname{35}
\expandafter\def\csname pn@opus.ctrl.out\endcsname{13{,}799}
\expandafter\def\csname pn@opus.ctrl1.ci\endcsname{[66.2, 89.1]}
\expandafter\def\csname pn@opus.ctrl1.cihi\endcsname{89.1}
\expandafter\def\csname pn@opus.ctrl1.cilo\endcsname{66.2}
\expandafter\def\csname pn@opus.ctrl1.cost\endcsname{1.83}
\expandafter\def\csname pn@opus.ctrl1.costmed\endcsname{1.26}
\expandafter\def\csname pn@opus.ctrl1.costsum\endcsname{82.3}
\expandafter\def\csname pn@opus.ctrl1.flippct\endcsname{---}
\expandafter\def\csname pn@opus.ctrl1.flips\endcsname{---}
\expandafter\def\csname pn@opus.ctrl1.job\endcsname{\texttt{cc-\allowbreak opus-\allowbreak hard45-\allowbreak nw}}
\expandafter\def\csname pn@opus.ctrl1.k\endcsname{36}
\expandafter\def\csname pn@opus.ctrl1.mcnemar\endcsname{---}
\expandafter\def\csname pn@opus.ctrl1.n\endcsname{45}
\expandafter\def\csname pn@opus.ctrl1.out\endcsname{15{,}984}
\expandafter\def\csname pn@opus.ctrl1.pct\endcsname{80.0}
\expandafter\def\csname pn@opus.ctrl1.reas\endcsname{4{,}916}
\expandafter\def\csname pn@opus.ctrl1.rows\endcsname{45}
\expandafter\def\csname pn@opus.ctrl1.steps\endcsname{34}
\expandafter\def\csname pn@opus.ctrl1.version\endcsname{2.1.263}
\expandafter\def\csname pn@opus.ctrl2.ci\endcsname{[63.7, 87.5]}
\expandafter\def\csname pn@opus.ctrl2.cihi\endcsname{87.5}
\expandafter\def\csname pn@opus.ctrl2.cilo\endcsname{63.7}
\expandafter\def\csname pn@opus.ctrl2.cost\endcsname{1.51}
\expandafter\def\csname pn@opus.ctrl2.costmed\endcsname{1.17}
\expandafter\def\csname pn@opus.ctrl2.costsum\endcsname{67.9}
\expandafter\def\csname pn@opus.ctrl2.flippct\endcsname{---}
\expandafter\def\csname pn@opus.ctrl2.flips\endcsname{---}
\expandafter\def\csname pn@opus.ctrl2.job\endcsname{\texttt{cc-\allowbreak opus-\allowbreak hard45-\allowbreak nw-\allowbreak k2}}
\expandafter\def\csname pn@opus.ctrl2.k\endcsname{35}
\expandafter\def\csname pn@opus.ctrl2.mcnemar\endcsname{1.00}
\expandafter\def\csname pn@opus.ctrl2.n\endcsname{45}
\expandafter\def\csname pn@opus.ctrl2.out\endcsname{12{,}777}
\expandafter\def\csname pn@opus.ctrl2.pct\endcsname{77.8}
\expandafter\def\csname pn@opus.ctrl2.reas\endcsname{5{,}927}
\expandafter\def\csname pn@opus.ctrl2.rows\endcsname{45}
\expandafter\def\csname pn@opus.ctrl2.steps\endcsname{32}
\expandafter\def\csname pn@opus.ctrl2.version\endcsname{2.1.263}
\expandafter\def\csname pn@opus.ctrl3.ci\endcsname{[63.7, 87.5]}
\expandafter\def\csname pn@opus.ctrl3.cihi\endcsname{87.5}
\expandafter\def\csname pn@opus.ctrl3.cilo\endcsname{63.7}
\expandafter\def\csname pn@opus.ctrl3.cost\endcsname{1.60}
\expandafter\def\csname pn@opus.ctrl3.costmed\endcsname{1.49}
\expandafter\def\csname pn@opus.ctrl3.costsum\endcsname{72.1}
\expandafter\def\csname pn@opus.ctrl3.flippct\endcsname{---}
\expandafter\def\csname pn@opus.ctrl3.flips\endcsname{---}
\expandafter\def\csname pn@opus.ctrl3.job\endcsname{\texttt{cc-\allowbreak opus-\allowbreak hard45-\allowbreak nw-\allowbreak k3}}
\expandafter\def\csname pn@opus.ctrl3.k\endcsname{35}
\expandafter\def\csname pn@opus.ctrl3.mcnemar\endcsname{1.00}
\expandafter\def\csname pn@opus.ctrl3.n\endcsname{45}
\expandafter\def\csname pn@opus.ctrl3.out\endcsname{14{,}930}
\expandafter\def\csname pn@opus.ctrl3.pct\endcsname{77.8}
\expandafter\def\csname pn@opus.ctrl3.reas\endcsname{5{,}345}
\expandafter\def\csname pn@opus.ctrl3.rows\endcsname{45}
\expandafter\def\csname pn@opus.ctrl3.steps\endcsname{39}
\expandafter\def\csname pn@opus.ctrl3.version\endcsname{2.1.263}
\expandafter\def\csname pn@opus.noshell.ci\endcsname{[61.3, 85.8]}
\expandafter\def\csname pn@opus.noshell.cihi\endcsname{85.8}
\expandafter\def\csname pn@opus.noshell.cilo\endcsname{61.3}
\expandafter\def\csname pn@opus.noshell.cost\endcsname{1.86}
\expandafter\def\csname pn@opus.noshell.costmed\endcsname{1.50}
\expandafter\def\csname pn@opus.noshell.costsum\endcsname{83.8}
\expandafter\def\csname pn@opus.noshell.flippct\endcsname{3.0}
\expandafter\def\csname pn@opus.noshell.flips\endcsname{4/135}
\expandafter\def\csname pn@opus.noshell.job\endcsname{\texttt{cc-\allowbreak opus-\allowbreak hard45-\allowbreak nw-\allowbreak c2ns}}
\expandafter\def\csname pn@opus.noshell.k\endcsname{34}
\expandafter\def\csname pn@opus.noshell.mcnemar\endcsname{0.50}
\expandafter\def\csname pn@opus.noshell.n\endcsname{45}
\expandafter\def\csname pn@opus.noshell.out\endcsname{16{,}734}
\expandafter\def\csname pn@opus.noshell.pct\endcsname{75.6}
\expandafter\def\csname pn@opus.noshell.reas\endcsname{10{,}031}
\expandafter\def\csname pn@opus.noshell.rows\endcsname{45}
\expandafter\def\csname pn@opus.noshell.steps\endcsname{26}
\expandafter\def\csname pn@opus.noshell.version\endcsname{2.1.263}
\expandafter\def\csname pn@opus.v1100.ci\endcsname{[61.3, 85.8]}
\expandafter\def\csname pn@opus.v1100.cihi\endcsname{85.8}
\expandafter\def\csname pn@opus.v1100.cilo\endcsname{61.3}
\expandafter\def\csname pn@opus.v1100.cost\endcsname{0.73}
\expandafter\def\csname pn@opus.v1100.costmed\endcsname{0.51}
\expandafter\def\csname pn@opus.v1100.costratio\endcsname{0.44}
\expandafter\def\csname pn@opus.v1100.costratio.med\endcsname{0.37}
\expandafter\def\csname pn@opus.v1100.costsum\endcsname{32.7}
\expandafter\def\csname pn@opus.v1100.flippct\endcsname{8.9}
\expandafter\def\csname pn@opus.v1100.flips\endcsname{12/135}
\expandafter\def\csname pn@opus.v1100.job\endcsname{\texttt{cc-\allowbreak opus-\allowbreak hard45-\allowbreak nw-\allowbreak v1100}}
\expandafter\def\csname pn@opus.v1100.k\endcsname{34}
\expandafter\def\csname pn@opus.v1100.mcnemar\endcsname{0.62}
\expandafter\def\csname pn@opus.v1100.n\endcsname{45}
\expandafter\def\csname pn@opus.v1100.out\endcsname{3{,}351}
\expandafter\def\csname pn@opus.v1100.outratio\endcsname{0.24}
\expandafter\def\csname pn@opus.v1100.pct\endcsname{75.6}
\expandafter\def\csname pn@opus.v1100.reas\endcsname{0}
\expandafter\def\csname pn@opus.v1100.rows\endcsname{45}
\expandafter\def\csname pn@opus.v1100.steps\endcsname{26}
\expandafter\def\csname pn@opus.v1100.version\endcsname{1.0.100}
\expandafter\def\csname pn@think.cc.ctok.off\endcsname{24{,}550}
\expandafter\def\csname pn@think.cc.ctok.on\endcsname{27{,}761}
\expandafter\def\csname pn@think.cc.delta.pp\endcsname{+2.2}
\expandafter\def\csname pn@think.cc.down\endcsname{5}
\expandafter\def\csname pn@think.cc.job.off\endcsname{\texttt{cc-\allowbreak qwen36-\allowbreak hard45-\allowbreak nw-\allowbreak nothink}}
\expandafter\def\csname pn@think.cc.n\endcsname{45}
\expandafter\def\csname pn@think.cc.off.k\endcsname{22}
\expandafter\def\csname pn@think.cc.off.mean\endcsname{0.256}
\expandafter\def\csname pn@think.cc.off.n\endcsname{87}
\expandafter\def\csname pn@think.cc.off.pct\endcsname{26}
\expandafter\def\csname pn@think.cc.on.k\endcsname{21}
\expandafter\def\csname pn@think.cc.on.mean\endcsname{0.233}
\expandafter\def\csname pn@think.cc.on.n\endcsname{90}
\expandafter\def\csname pn@think.cc.on.pct\endcsname{23}
\expandafter\def\csname pn@think.cc.p\endcsname{.77}
\expandafter\def\csname pn@think.cc.pfull\endcsname{0.774}
\expandafter\def\csname pn@think.cc.same\endcsname{33}
\expandafter\def\csname pn@think.cc.steps.off\endcsname{126}
\expandafter\def\csname pn@think.cc.steps.on\endcsname{103.5}
\expandafter\def\csname pn@think.cc.up\endcsname{7}
\expandafter\def\csname pn@think.hy4.cny.off\endcsname{2.14}
\expandafter\def\csname pn@think.hy4.cny.on\endcsname{2.86}
\expandafter\def\csname pn@think.hy4.ctok.off\endcsname{15{,}001}
\expandafter\def\csname pn@think.hy4.ctok.on\endcsname{43{,}189}
\expandafter\def\csname pn@think.hy4.delta.pp\endcsname{$-$11.1}
\expandafter\def\csname pn@think.hy4.down\endcsname{9}
\expandafter\def\csname pn@think.hy4.drop.pp\endcsname{11}
\expandafter\def\csname pn@think.hy4.job.off\endcsname{\texttt{cc-\allowbreak hy4-\allowbreak hard45-\allowbreak nw-\allowbreak nothink}}
\expandafter\def\csname pn@think.hy4.job.on\endcsname{\texttt{cc-\allowbreak hy4-\allowbreak hard45-\allowbreak nw-\allowbreak r}}
\expandafter\def\csname pn@think.hy4.mcnemar\endcsname{.27}
\expandafter\def\csname pn@think.hy4.n\endcsname{45}
\expandafter\def\csname pn@think.hy4.off.k\endcsname{18}
\expandafter\def\csname pn@think.hy4.off.mean\endcsname{0.400}
\expandafter\def\csname pn@think.hy4.off.n\endcsname{45}
\expandafter\def\csname pn@think.hy4.off.pct\endcsname{40}
\expandafter\def\csname pn@think.hy4.on.k\endcsname{23}
\expandafter\def\csname pn@think.hy4.on.mean\endcsname{0.511}
\expandafter\def\csname pn@think.hy4.on.n\endcsname{45}
\expandafter\def\csname pn@think.hy4.on.pct\endcsname{51}
\expandafter\def\csname pn@think.hy4.outk.off\endcsname{17.5}
\expandafter\def\csname pn@think.hy4.outk.on\endcsname{43.9}
\expandafter\def\csname pn@think.hy4.outratio\endcsname{0.40}
\expandafter\def\csname pn@think.hy4.p\endcsname{.27}
\expandafter\def\csname pn@think.hy4.pfull\endcsname{0.267}
\expandafter\def\csname pn@think.hy4.same\endcsname{32}
\expandafter\def\csname pn@think.hy4.steps.off\endcsname{90}
\expandafter\def\csname pn@think.hy4.steps.on\endcsname{75}
\expandafter\def\csname pn@think.hy4.up\endcsname{4}
\expandafter\def\csname pn@think.mini.ctok.off\endcsname{20{,}582}
\expandafter\def\csname pn@think.mini.ctok.on\endcsname{25{,}198}
\expandafter\def\csname pn@think.mini.delta.pp\endcsname{$-$11.1}
\expandafter\def\csname pn@think.mini.down\endcsname{10}
\expandafter\def\csname pn@think.mini.drop.pp\endcsname{11}
\expandafter\def\csname pn@think.mini.job.off\endcsname{\texttt{mini-\allowbreak qwen36-\allowbreak hard45-\allowbreak nw-\allowbreak nothink}}
\expandafter\def\csname pn@think.mini.n\endcsname{45}
\expandafter\def\csname pn@think.mini.off.k\endcsname{18}
\expandafter\def\csname pn@think.mini.off.mean\endcsname{0.200}
\expandafter\def\csname pn@think.mini.off.n\endcsname{90}
\expandafter\def\csname pn@think.mini.off.pct\endcsname{20}
\expandafter\def\csname pn@think.mini.on.k\endcsname{28}
\expandafter\def\csname pn@think.mini.on.mean\endcsname{0.311}
\expandafter\def\csname pn@think.mini.on.n\endcsname{90}
\expandafter\def\csname pn@think.mini.on.pct\endcsname{31}
\expandafter\def\csname pn@think.mini.p\endcsname{.04}
\expandafter\def\csname pn@think.mini.pfull\endcsname{0.039}
\expandafter\def\csname pn@think.mini.same\endcsname{33}
\expandafter\def\csname pn@think.mini.steps.off\endcsname{98}
\expandafter\def\csname pn@think.mini.steps.on\endcsname{106.5}
\expandafter\def\csname pn@think.mini.up\endcsname{2}
\expandafter\def\csname pn@think.oc.ctok.off\endcsname{15{,}949.5}
\expandafter\def\csname pn@think.oc.ctok.on\endcsname{14{,}018}
\expandafter\def\csname pn@think.oc.delta.pp\endcsname{+3.4}
\expandafter\def\csname pn@think.oc.down\endcsname{5}
\expandafter\def\csname pn@think.oc.job.off\endcsname{\texttt{oc-\allowbreak qwen36-\allowbreak hard45-\allowbreak nw-\allowbreak nothink}}
\expandafter\def\csname pn@think.oc.n\endcsname{44}
\expandafter\def\csname pn@think.oc.off.k\endcsname{16}
\expandafter\def\csname pn@think.oc.off.mean\endcsname{0.182}
\expandafter\def\csname pn@think.oc.off.n\endcsname{86}
\expandafter\def\csname pn@think.oc.off.pct\endcsname{18}
\expandafter\def\csname pn@think.oc.on.k\endcsname{15}
\expandafter\def\csname pn@think.oc.on.mean\endcsname{0.148}
\expandafter\def\csname pn@think.oc.on.n\endcsname{88}
\expandafter\def\csname pn@think.oc.on.pct\endcsname{15}
\expandafter\def\csname pn@think.oc.p\endcsname{.77}
\expandafter\def\csname pn@think.oc.pfull\endcsname{0.774}
\expandafter\def\csname pn@think.oc.same\endcsname{32}
\expandafter\def\csname pn@think.oc.steps.off\endcsname{78.5}
\expandafter\def\csname pn@think.oc.steps.on\endcsname{56}
\expandafter\def\csname pn@think.oc.up\endcsname{7}
\expandafter\def\csname pn@think.outratio\endcsname{1.23}
\expandafter\def\csname pn@think.outratio.means\endcsname{1.19}
\expandafter\def\csname pn@think.share.cc\endcsname{82.5}
\expandafter\def\csname pn@think.share.cc.outk\endcsname{51.2}
\expandafter\def\csname pn@think.share.n\endcsname{444}
\expandafter\def\csname pn@think.share.oc\endcsname{82.9}
\expandafter\def\csname pn@think.share.oc.outk\endcsname{43.2}
\makeatother


==> numbers_ctx.tex <==
\makeatletter
\@ifundefined{pn}{\DeclareRobustCommand{\pn}[1]{\csname pn@#1\endcsname}}{}
\expandafter\def\csname pn@ctx.dsflash.CC.first.k\endcsname{17.8}
\expandafter\def\csname pn@ctx.dsflash.CC.intercept.k\endcsname{22.2}
\expandafter\def\csname pn@ctx.dsflash.CC.n\endcsname{45}
\expandafter\def\csname pn@ctx.dsflash.CC.reason.step\endcsname{187}
\expandafter\def\csname pn@ctx.dsflash.CC.slope\endcsname{1{,}308}
\expandafter\def\csname pn@ctx.dsflash.OC.first.k\endcsname{8.0}
\expandafter\def\csname pn@ctx.dsflash.OC.intercept.k\endcsname{8.9}
\expandafter\def\csname pn@ctx.dsflash.OC.n\endcsname{45}
\expandafter\def\csname pn@ctx.dsflash.OC.reason.step\endcsname{110}
\expandafter\def\csname pn@ctx.dsflash.OC.slope\endcsname{1{,}116}
\expandafter\def\csname pn@ctx.dsflash.mini.first.k\endcsname{1.6}
\expandafter\def\csname pn@ctx.dsflash.mini.intercept.k\endcsname{4.1}
\expandafter\def\csname pn@ctx.dsflash.mini.n\endcsname{45}
\expandafter\def\csname pn@ctx.dsflash.mini.reason.step\endcsname{116}
\expandafter\def\csname pn@ctx.dsflash.mini.slope\endcsname{1{,}037}
\expandafter\def\csname pn@ctx.glmflash.CC.first.k\endcsname{17.1}
\expandafter\def\csname pn@ctx.glmflash.CC.intercept.k\endcsname{32.1}
\expandafter\def\csname pn@ctx.glmflash.CC.n\endcsname{45}
\expandafter\def\csname pn@ctx.glmflash.CC.reason.step\endcsname{82}
\expandafter\def\csname pn@ctx.glmflash.CC.slope\endcsname{937}
\expandafter\def\csname pn@ctx.glmflash.OC.first.k\endcsname{7.6}
\expandafter\def\csname pn@ctx.glmflash.OC.intercept.k\endcsname{11.6}
\expandafter\def\csname pn@ctx.glmflash.OC.n\endcsname{45}
\expandafter\def\csname pn@ctx.glmflash.OC.reason.step\endcsname{10}
\expandafter\def\csname pn@ctx.glmflash.OC.slope\endcsname{681}
\expandafter\def\csname pn@ctx.glmflash.mini.first.k\endcsname{1.4}
\expandafter\def\csname pn@ctx.glmflash.mini.intercept.k\endcsname{8.7}
\expandafter\def\csname pn@ctx.glmflash.mini.n\endcsname{45}
\expandafter\def\csname pn@ctx.glmflash.mini.reason.step\endcsname{26}
\expandafter\def\csname pn@ctx.glmflash.mini.slope\endcsname{648}
\makeatother

